Derangements and the $p$-adic incomplete gamma function

We introduce a $p$-adic analogue of the incomplete gamma function. We also introduce quantities ($m$-values) associated to a function on natural numbers and prove a new characterization of $p$-adic continuity for functions with $p$-integral $m$-values. Combinatorial interpretations for the integral values of the incomplete gamma function and functions with $m$-values zero or one are obtained, which show that these functions count derangements in generalized symmetric groups and permutations with restricted cycle lengths.

==> ig-header.tex <==
% LaTeX header file for Derangements and the $p$-adic incomplete gamma function

% Imports
\usepackage[margin=1.4in]{geometry}
%\RequirePackage{setspace} % line spacing
\RequirePackage{tikz,tikz-cd} % diagrams
\usepackage{xcolor}
\definecolor{myblue}{HTML}{2098df} 
\definecolor{myotherblue}{HTML}{0d83f2} 
\definecolor{mygreen}{HTML}{3BC4BD} 
\definecolor{mydarkerblue}{HTML}{3B87C4} 
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=myotherblue, 
    citecolor=mygreen, 
    urlcolor=myblue,
}
%\urlstyle{tt}
%\usepackage{bbold}
%\usepackage{dsfont}
\usepackage{xifthen}
\usepackage{amssymb}
\usepackage{enumerate} % customize numbering
\usepackage{mathtools}
%\usepackage{newtxmath}
%\usepackage{unicode-math}
\allowdisplaybreaks

\pagestyle{empty}
    
\mathtoolsset{showonlyrefs} % Only show equation numbers for referenced equations

% \mathbb, \mathfrak
\newcommand{\NN}{\mathbb N}
% positive integers
\newcommand{\NNpos}{\mathbb N^{>0}}
\newcommand{\ZZ}{\mathbb Z}
\newcommand{\QQ}{\mathbb Q}
\newcommand{\RR}{\mathbb R}
\newcommand{\CC}{\mathbb C}
\newcommand{\FF}{\mathbb F}

% Misc symbols/functions
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\isom}{\cong}
\DeclareMathOperator{\lcm}{lcm}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\note}[1]{{\color{magenta} [{#1}]}}
\newcommand{\crp}[2]{d^{#1}_{#2}} % cycle restricted permutation
\renewcommand{\Re}{\mathrm{Re}}
%\newcommand{\LA}{\mathrm{LA}}
%\newcommand{\LA}{\EGFalg{}^{\mathrm{la}} }
\newcommand{\charfn}[1]{\chi_{#1}} % characteristic function

% Latex modifiers
\newcommand{\ds}{\displaystyle}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

%\newcommand{\defn}[1]{\textsf{#1}}
\newcommand{\defn}[1]{\emph{#1}}

% Environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem*{prop*}{Proposition}
\newtheorem{unlabeled}[theorem]{}
\newtheorem{noheadsubsection}[equation]{}

\theoremstyle{definition} % No italics in this environment
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{warning}{Warning}
\newtheorem*{warning*}{Warning}
\newtheorem*{example*}{Example}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}

\theoremstyle{remark} % No italics in this environment
\newtheorem{innerobservation}{Observation} % Theorem environment with custom number
\newenvironment{observation}[1]
  {\renewcommand\theinnerobservation{#1}\innerobservation}
  {\endinnerobservation}
\newtheorem{case}{Case}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem*{questions*}{Questions}
\newtheorem{question}{Question}
\newtheorem*{problem}{Problem}

% Definitions:
\newcommand{\ul}{\underline}
\newcommand{\seq}[1][]{% generic sequence
    %\ifthenelse{\isempty{#1}{}}{{s}}{s({#1})}%
    \ifthenelse{\isempty{#1}{}}{{s}}{s_{#1}}%
}
\newcommand{\findiff}[1][]{% finite differences
    \ifthenelse{\isempty{#1}{}}{{c}}{c({#1})}%
}
\newcommand{\ddtwo}[2]{{#2}_{#1}} % higher divided difference
\newcommand{\dd}[2]{\delta_{#1}{#2}} % higher divided difference
\newcommand{\alg}[1]{\langle #1\rangle} % sequence from pole 
\newcommand{\poly}{f} % generic polynomial 
\newcommand{\norm}[1][]{% generic norm
    \ifthenelse{\isempty{#1}{}}
        {\left\lVert \,\cdot\, \right\rVert}%
        {\left\lVert#1\right\rVert}%
}
\newcommand{\Int}[1]{I^{#1}}
\newcommand*{\callig}{\fontfamily{calligra}\selectfont}
\newcommand*{\zapf}{\fontfamily{pzc}\selectfont}
\DeclareTextFontCommand{\textcg}{\callig}
\DeclareTextFontCommand{\textzc}{\zapf}
%\newcommand{\INT}[1]{\textup{\textbf{Int}}^{#1}}
\newcommand{\INT}[1]{{\mathcal{I}}^{#1}}
\newcommand{\stirone}[2]
    {\left[ \begin{matrix} 
            {#1} \\ {#2}
    \end{matrix} \right]}
\newcommand{\Ei}{\operatorname{Ei}} % Euler integral
\newcommand{\sms}[1]{\langle #1\rangle} % smooth sequence
\newcommand{\seqtwo}[1][]{% another generic sequence
    \ifthenelse{\isempty{#1}{}}{{t}}{t({#1})}%
}


\newcommand{\embedding}[1][]{% embedding corresponding to a place
    \ifthenelse{\isempty{#1}{}}
    {i}
    {i_{#1}} 
    }
\newcommand{\icg}[1][]{
    % incomplete gamma function
    % \icg[s,z] = Gamma(s,z), Gamma(s,0) = Gamma(s)
    \ifthenelse{\isempty{#1}{}}
        {\Gamma(s,z)}%
        {\Gamma(#1)}%
}

\newcommand{\icgo}[3]{
    % incomplete gamma function without period
    % \icgo{p}{s}{u} = Gamma_p(s,u)
    \gamma_{#1}(#2,#3)
}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}

\newcommand{\hall}[1]{H_{#1}} % Hall sequence
\newcommand
    {\mgamma}[1]{\Gamma_{#1}} % Morita {#1}-adic gamma function 
\newcommand{\valn}[1][]{% valuation corresponding to a place
    \ifthenelse{\isempty{#1}{}}
    {v}
    {v_{#1}} 
    }
\newcommand{\derangements}[1]{d_{#1}} % number of derangements of degree n
\newcommand{\arrangements}[1]{a_{#1}} % number of arrangements of degree $n$
%\newcommand{\cderangements}[2]{d^{(#1)}_{#2}} % number of cyclic derangements 
\newcommand{\dr}[2]{d_{#2}^{\,({#1})}} % number of cyclic derangements
%\newcommand{\EGFalg}[1]{E_0(#1)} % power series with EGF-coeffs going to zero. 
%\newcommand{\EGFalg}[1]{#1 \{ X \}^\mathrm{exp}} % power series with EGF-coeffs going to zero. 
\newcommand{\EGFalg}[1]{V} % power series with EGF-coeffs going to zero. 
\newcommand{\Tatealg}[1]{#1 \{ X \}} % power series with OGF-coeffs going to zero. 
\newcommand{\TatealgX}[2]{#1 \{ #2 \}} % power series with OGF-coeffs going to zero. 
\newcommand{\RIGIDalg}[2]{A_{#1}(#2)} % power series with EGF-coeffs going to zero. 
\newcommand{\RIGIDalgcl}[2]{A_{#1}^{\mathrm{cl}}(#2)} % power series with EGF-coeffs going to zero. 
%\newcommand{\gs}[2]{\langle {#1} \rangle_{#2}}
\newcommand{\gs}[2]{a(#1,#2)}
%\newcommand{\gsp}[2]{\tilde{a}(#1,#2)}
\newcommand{\gsp}[2]{a_p(#1,#2)}
\newcommand{\algclosure}[1]{\overbar{#1}}


